Large Language Models for Power Scheduling: A User-Centric Approach

While traditional optimization and scheduling schemes are designed to meet fixed, predefined system requirements, future systems are moving toward user-driven approaches and personalized services, aiming to achieve high quality-of-experience (QoE) and flexibility. This challenge is particularly pronounced in wireless and digitalized energy networks, where users' requirements have largely not been taken into consideration due to the lack of a common language between users and machines. The emergence of powerful large language models (LLMs) marks a radical departure from traditional system-centric methods into more advanced user-centric approaches by providing a natural communication interface between users and devices. In this paper, for the first time, we introduce a novel architecture for resource scheduling problems by constructing three LLM agents to convert an arbitrary user's voice request (VRQ) into a resource allocation vector. Specifically, we design an LLM intent recognition agent to translate the request into an optimization problem (OP), an LLM OP parameter identification agent, and an LLM OP solving agent. To evaluate system performance, we construct a database of typical VRQs in the context of electric vehicle (EV) charging. As a proof of concept, we primarily use Llama 3 8B. Through testing with different prompt engineering scenarios, the obtained results demonstrate the efficiency of the proposed architecture. The conducted performance analysis allows key insights to be extracted. For instance, having a larger set of candidate OPs to model the real-world problem might degrade the final performance because of a higher recognition/OP classification noise level. All results and codes are open source.

==> Figures/gpt-system.tex <==
\begin{tikzpicture}
\def\pad{1.3}
% Nodes
\node (OR) {};
\node[basicblock,draw=user-request-primary,fill=user-request-gray, right = \pad of OR] (classify) {Classifier};
\node[basicblock,draw=user-request-primary,fill=user-request-gray, right = \pad of classify] (parse) {Parser};
\node[above = 10pt of parse, font=\scriptsize,text=black!50!white] (CT) {current time};
\node[right = \pad of parse] (END) {};

% Arrows
\draw[myarrow] (OR) to [edge label=user request, font=\scriptsize, text width=3em, align=center] (classify);
\draw[myarrow] ([yshift=5pt]classify.east) --  ([yshift=5pt]parse.west) node [midway,above,draw=none,font=\scriptsize, text width=3em, align=center] {user request};
\draw[myarrow] ([yshift=-5pt]classify.east) -- ([yshift=-5pt]parse.west) node [midway,below,draw=none,font=\scriptsize, text width=3em, align=center] {OP/OCP class};
\draw[myarrow] (parse) -- (END) node [midway,above,draw=none,font=\scriptsize, text width=3em, align=center] {function calling};
\draw[myarrow,dashed,shorten <=1] (classify.south) -- ([yshift=-18pt]classify.south) -- node [midway,below,draw=none,font=\scriptsize, text width=10em, align=center] {knowledge + function} ([yshift=-18pt]parse.south) -- (parse.south);
\draw[myarrow,draw=black!50!white] (CT) -- (parse);
\end{tikzpicture}

==> Figures/sh-context.tex <==
\begin{tikzpicture}
    \def\pad{1.3}
    \node (OR) {};
    \node[basicblockshadow, draw, fill=white, right = \pad of OR] (STT) {STT};
    \node[basicblock,draw=black, right = \pad of STT] (classify) {Classifier};
    \node[basicblock,draw=black, right = \pad of classify] (parse) {Parser};
    \node[above = 10pt of parse, font=\tiny,text=black!50!white] (CT) {current time};
    %\node[basicblock,draw=user-request-primary,fill=user-request-gray, right = \pad of OR,text width=5em] (gpt) {GPT-based system};
    %\draw[rounded corners, color=cyan!60, dash pattern=on 8pt off 3pt, line width=1.2pt] (gpt)++(\pad+2.5,1.2) to ++(\pad+2.5,0) to ++(0,-2.4)  --  ++(-\pad-2.5,0) node [font=\scriptsize, midway, above, fill=white] {Electrical installation} -- cycle;

    \node[basicblockshadow,draw=json-primary,fill=json-gray, right = \pad of parse, text width=4em] (SM) {Smart Meter + Solver};
    \node[basicblockshadow,draw=openai-primary,fill=openai-gray, right = \pad of SM] (SHA) {SH Appliance};
    %\node[right = \pad of EVC] (END) {};
    
    
    \draw[myarrow] (STT) to [edge label=text request, font=\tiny, text width=3em, align=center] (classify);
    \draw[myarrow] ([yshift=5pt]classify.east) --  ([yshift=5pt]parse.west) node [midway,above,draw=none,font=\tiny, text width=3em, align=center] {text request};
    \draw[myarrow] ([yshift=-5pt]classify.east) -- ([yshift=-5pt]parse.west) node [midway,below,draw=none,font=\tiny, text width=3em, align=center] {OP/OCP class};
    \draw[myarrow,dashed,shorten <=1] (classify.south) -- ([yshift=-18pt]classify.south) -- node [midway,below,draw=none,font=\tiny, text width=10em, align=center, name=l] {knowledge + function} ([yshift=-18pt]parse.south) -- (parse.south);
    \draw[myarrow,draw=black!50!white] (CT) -- (parse);
    
    \draw[myarrow] (OR) -- (STT) node [midway,above,draw=none,font=\tiny, text width=3em, align=center] {vocal request};
    \draw[myarrow] (parse) -- (SM) node [midway,above,draw=none,font=\tiny, text width=3em, align=center] {function calling};
    \draw[myarrow] ([yshift=5pt]SM.east) -- ([yshift=5pt]SHA.west) node [midway,above,draw=none,font=\tiny, text width=3em, align=center] {power scheduling};
    \draw[myarrow] ([yshift=-5pt]SHA.west) -- ([yshift=-5pt]SM.east) node [midway,below,draw=none,font=\tiny, text width=4em, align=center] {data};
    
    
    
    \begin{scope}[on background layer]
    	\node[basicblockshadow,draw=user-request-primary,fill=user-request-gray,inner xsep=7.5pt,inner ysep=2pt,fit=(classify)(parse)(l)(CT),label={[anchor=north west,font=\tiny\bfseries\color{user-request-primary},outer sep=2pt]north west:GPT-based system}]{};
    \end{scope}
\end{tikzpicture}


==> Figures/tikz-config <==
\tikzset{every picture/.style={/utils/exec={\sffamily},font=\fontsize{6pt}{11pt}\selectfont}}
\tikzset{
    basicblock/.style={
        rectangle,
        rounded corners=5,
        inner sep=6pt,
        text centered,
        minimum width=1.6cm,
        minimum height=.8cm,
        font = \normalsize,
        line width=1.5pt
    }
}

\tikzset{
	basicblockshadow/.style={
	rectangle,
	rounded corners=5,
	inner sep=6pt,
	%draw=black,  % Border color
	blur shadow={
		shadow blur steps=5,
		shadow blur radius=1pt, 
		shadow xshift=3pt,
		shadow yshift=-3pt,
		shadow opacity=22
	},  % Shadow
	text centered,
	minimum width=1.6cm,
	minimum height=.8cm,
	node font = \normalsize,
	line width=1.5pt
	}
}

\tikzset{
	myarrow/.style={
		-{Latex[round]},
		thick
	}
}

